CAT: Causal Audio Transformer for Audio Classification

The attention-based Transformers have been increasingly applied to audio classification because of their global receptive field and ability to handle long-term dependency. However, the existing frameworks which are mainly extended from the Vision Transformers are not perfectly compatible with audio signals. In this paper, we introduce a Causal Audio Transformer (CAT) consisting of a Multi-Resolution Multi-Feature (MRMF) feature extraction with an acoustic attention block for more optimized audio modeling. In addition, we propose a causal module that alleviates over-fitting, helps with knowledge transfer, and improves interpretability. CAT obtains higher or comparable state-of-the-art classification performance on ESC50, AudioSet and UrbanSound8K datasets, and can be easily generalized to other Transformer-based models.

==> sections/archived.tex <==
% In patch-based audio models\cite{chen2022hts,gong2021ast,koutini2021efficient}, the input spectrogram is divided into patches of amplitudes, as in ViT, the image is divided into patches of pixels. Then the patches are served as sequential input to the \Transformer models. However, different from images where the x and y axis shares the same meaning (i.g. the location of a pixel), in audio spectrograms, x-axis usually represents time while y-axis represents discrete frequency. Such differences break the two underlying assumptions in images: (1) one pixel value usually belongs to one object, but one amplitude in the spectrogram may result from the accumulation of multiple sources of sound. (2) Frequencies have a periodic nature and they are non-locally distributed. For instance, neighboring amplitude along the frequency axis can hardly be grouped together for representing the local features of an object.  (3) Different from images where pixel values contain basically all information about an image. Acoustic features can be captured from different angles, such as raw spectrogram, mel-spectrogram, waveforms and etc. 
% As a result, we need different representation and modelling than local patches commonly used for images.

% Discovering and eliminating spurious features is a goal for almost all deep audio models, including the SOTA Transformer-based audio models. A model with a large number of spurious features may lead to unintended effects, such as over-fitting, poor transferring robustness, or being susceptible to adversarial attacks. Although extended from ViT, unfortunately, there still exists a performance gap when applying remedies from the image domain. For example, while mixup\cite{zhang2017mixup} reduced the test error to half of its original value on CIFAR10\cite{krizhevsky2009learning} with the corrupted label, a direct extension as in \cite{gong2021ast, koutini2021efficient} only obtained around $15\%$ improved on ESC50\cite{piczak2015dataset} with the same percentage of the corrupted label. In addition, some of the most popular methods for eliminating spurious features are based on the availability of interpretable visual features\cite{chung2019slice}, human-annotated dataset\cite{plumb2021finding}, and strong domain knowledge and assumptions in vision tasks\cite{singla2021salient}, leaving designing non-adhoc algorithms for audio data imperative.

% \textbf{(2) Lack of explicit metric in measuring spurious features in the inference.} 
% Discovering and eliminating spurious features is a goal for almost of audio-related tasks. The end-to-end structure of popular audio classification models makes it difficult to directly understand, measure, and justify the features extracted in the models and their predictions. This may lead to unintended effects, such as over-fitting, capturing spurious features, or being susceptible to adversarial attacks. Although inherited the main structure from ViT, methods in the image domain can hardly be transferred to existing attention-based audio models due to their strong dependence on domain knowledge and specific model structures. Most of the prior works depend on a possible list of the visual spurious feature\cite{}, theoretically robust visual feature detector\cite{} or associate visual attributes to the predictive tasks\cite{}.
% Consequently, we argue that an explicit, domain-independent measurement of spurious features is desired. 
%




% related work

% scholars adapted the audio frameworks to a \Transformer backbone\cite{vaswani2017attention}, obtaining state-of-the-art (SOTA) performance in the end-to-end training, such as MBT\cite{nagrani2021attention}, PaSST\cite{koutini2021efficient}, HTS-AT\cite{chen2022hts} and etc.\Transformer is introduced in 2017, in the context of sequential modelling in NLP. It is first extended to the audio domain in the Audio Spectrogram Transformer (AST) \cite{gong2021ast} paper, where the spectrogram is used as the input into a ViT\cite{dosovitskiy2020image} framework. Multiple subsequent works focus on the efficiency and the complexity of the model, such as PaSST \cite{koutini2021efficient} which designed the patch-out mechanism, and HTS-AT\cite{chen2022hts} that adopts a similar structure to the SWIN\cite{liu2021swin}. Another line of research focused on pretraining and multi-modality models. MBT\cite{nagrani2021attention} introduces an audiovisual fusion procedure, PLSA\cite{gong2021psla} took a holistic view from pertaining, sampling and aggregation, then proposed a model-agnostic framework to improve the performance in the audio-tagging task. In this paper, we also adopt a SWIN-like structure with less computation and memory requirements. Different from these existing works, \ourmodel features a tailored design for the audio signal, together with a causal framework that eliminates the spurious feature, reduces over-fitting, and improves transfer robustness. 

% 
  % In recent years, causal models are increasingly used in improving feature qualities, especially in generative models\cite{yang2021causalvae, reddy2022causally,suter2019robustly, nangi2021counterfactuals}. CausalVAE\cite{yang2021causalvae} demonstrates that modelling causality among generating factors significantly encourages the learning of representative features. \cite{suter2019robustly,nangi2021counterfactuals} reasons about counterfactual information and proved that causal formulation improves knowledge transfer across different domains. In this paper, we derive a framework on top of \cite{wang2021desiderata}, where the author associated the rules of thumbs in representation learning with its rigorous causal implementation. Instead of approaching unobserved confounder $C$ using probabilistic factor models, we consider under the context of audio classification and relax the constraint between $X$ and $Z$ by introducing a reconstruction layer and minimizing the reconstruction error and pairing it with a causal loss.

  % Different from image-related tasks where almost all information is contained within pixels, the majority of models use the spectrogram as input. However, features from acoustic knowledge or engineering expertise may not perfectly suit the specific tasks or networks. Considering the power of global attention brought by \Transformer, we propose a multi-resolution and multi-filter design for audio signal.

  % In each spectrogram, the patches are first sampled along the time axis and then the frequency axis so that each patch maintains the locality in time to a maximal extent. We then concatenate patches from different resolutions within the same window. Each patch is equipped with a disentangled positional encoding similar to \cite{koutini2021efficient}, i.e, we generate individual encoding vectors in time, frequency and resolution, and add them to the patches. The patches are then sent to a hierarchical structure consisting of Patch-Merge Layers and SWIN Transformer Blocks\cite{liu2021swin} as shown in Figure~\ref{fig:training}. Note that although we expand the input from a single spectrogram to a set of spectrograms in different resolutions, the computational complexity is not changed due to the window mechanism. 



% \noindent\textbf{Acoustic attention: pairwise attention across multi-resolution patches and multi-filter across attention heads.}
% We first enrich the acoustic features by extracting spectrograms under different resolutions in Figure~\ref{fig:multi-resolution}. The intuition comes from the fact that frequency resolution is much more important in the lower frequency ranges, however, high resolution in frequency means sacrificing in the time domain, due to the nature of 2D FFT. While both of them are considered critical for acoustic modeling, we propose multi-resolution input, which resembles the intuition\cite{zhu2018learning, grais2018multi}, but is adapted to the Transformer backbone to allow the study of pair-wise associations between pieces of audio signals. This way, we could not only enforce feature studies at the same scale but also allow dynamic learning across levels of abstraction.

% In each spectrogram, the patches are first sampled along the time axis and then the frequency axis so that each patch maintains the locality in time to a maximal extent. We then concatenate patches from different resolutions within the same window. Each patch is equipped with a disentangled positional encoding similar to \cite{koutini2021efficient}, i.e, we generate individual encoding vectors in time, frequency and resolution, and add them to the patches. The patches are then sent to a hierarchical structure consisting of Patch-Merge Layers and SWIN Transformer Blocks\cite{liu2021swin} as shown in Figure~\ref{fig:training}. Note that although we expand the input from a single spectrogram to a set of spectrograms in different resolutions, the computational complexity is not changed due to the window mechanism. 



% \noindent\textbf{Acoustic attention: pairwise attention across multi-resolution patches and multi-filter across attention heads.}
% We first enrich the acoustic features by extracting spectrograms under different resolutions in Figure~\ref{fig:multi-resolution}. The intuition comes from the fact that frequency resolution is much more important in the lower frequency ranges, however, high resolution in frequency means sacrificing in the time domain, due to the nature of 2D FFT. While both of them are considered critical for acoustic modeling, we propose multi-resolution input, which resembles the intuition\cite{zhu2018learning, grais2018multi}, but is adapted to the Transformer backbone to allow the study of pair-wise associations between pieces of audio signals. This way, we could not only enforce feature studies at the same scale but also allow dynamic learning across levels of abstraction.


% \noindent\textbf{Patch sampling and disentangled positional encoding.} 
% In each spectrogram, the patches are first sampled along the time axis and then the frequency axis so that each patch maintains the locality in time to a maximal extent. We then concatenate patches from different resolutions within the same window. Each patch is equipped with a disentangled positional encoding similar to \cite{koutini2021efficient}, i.e, we generate individual encoding vectors in time, frequency and resolution, and add them to the patches. The patches are then sent to a hierarchical structure consisting of Patch-Merge Layers and SWIN Transformer Blocks\cite{liu2021swin} as shown in Figure~\ref{fig:training}. Note that although we expand the input from a single spectrogram to a set of spectrograms in different resolutions, the computational complexity is not changed due to the window mechanism. 

% \noindent\textbf{Pairwise attention across patches in multi-resolution and multi-filter across attention heads.}
% We first enrich the acoustic features by extracting spectrograms under different resolutions in Figure~\ref{fig:multi-resolution}. The intuition comes from the fact that frequency resolution is much more important in the lower frequency ranges, however, high resolution in frequency means sacrificing in the time domain, due to the nature of 2D FFT. While both of them are considered critical for acoustic modeling, we propose multi-resolution input, which resembles the intuition\cite{zhu2018learning, grais2018multi}, but is adapted to the Transformer backbone to allow the study of pair-wise associations between pieces of audio signals. This way, we could not only enforce feature studies at the same scale but also allow dynamic learning across levels of abstraction.

% In addition, we make use of the multi-head design of the attention module by feeding different head spectrograms created by different filters. In this paper, we use the Mel-filtered and the unfiltered spectrogram.


%\xinyu{verbose, i rewrite the problem definition, please feel free to ignore.}
%\textbf{(1) Audio signals inherently differ from images, thus they require a meticulously-designed structure following their own patterns.} 
%\xinyu{The commonly used acoustic representations utilize different time-frequency transformations, and contain acoustic semantics of various scales and different granularities~\cite{chen2022hts,gong2021ast,koutini2021efficient}, thus, cannot be effectively captured by image patch embedding and conventional attentions used in ViTs~\cite{dosovitskiy2020image}.}


%
%\textbf{(2) There is a lack of non ad hoc methods for eliminating spurious features in audio data.}
%\xinyu{We observe that the similar models (e.g. resnet~\cite{krizhevsky2009learning}) and techniques (e.g. mixup~\cite{zhang2017mixup}) are more prone to over-fitting and less generalizable in acoustic domain. Feature selection and representation learning is an important topic for computer vision~\cite{chung2019slice,plumb2021finding,singla2021salient} but often overlooked in acoustic modeling tasks.}
% which {\color{red}incorporates a multi-resolution and multi-filter modeling ?--JY} tailored for audio signals and a causal loss that directly measures and improves the quality of inferred features in the latent space. \modelshortcut samples patches only along the time-axis, with disentangled time and frequency positional embedding. Then, the multi-resolution inputs are scattered across different attention heads while different filtered inputs are concatenated sequentially. 

% Note that both modules generalize well to conventional transformer backbones, we illustrate the overall structure with SWIN transformer backbone, which is also the current SOTA acoustic model as shown in . 
% The input for the model is patches extracted from the original audio spectrograms and filtered audio spectrograms in different resolutions. Then we encode the patches with disentangled time, frequency and resolution information. The input patches are sent to a hierarchical structure with shifted windows as in \cite{liu2021swin, chen2022hts}. We choose such a design because it has a state-of-the-art model performance on audio classification/tagging task across various dataset. In addition, the shifted-window mechanism improves both computation complexity and generalization by establishing the hierarchy. We then build a reconstruction layer in parallel to classification layer using the inferred representation from the hierarchical structure. Finally, we optimize the reconstruction error, causal loss, and classification objective. 
% \xinyu{we first introduce our acoustic transformer with multi-scale patching and multi-filter attention heads (section XX). Then we will present the causal loss (section XX).Note that both modules generalize well to conventional transformer backbones, we illustrate the overall structure with SWIN transformer backbone, which is also the current SOTA acoustic model.(Fig 1)}
%
% \subsection{Transformer For Acoustic Modeling}
% \label{sec:model-multi}
% It is not trivial to apply a commonly used vision transformer to the acoustic domain. We first carefully design the patch embedding strategies to ensure the full coverage of information at different scales and granularity. We then propose multi-resolution multi-filter attention to model the acoustic semantics.




% We propose to append multi-scale patch embedding to patch features. We first sample the original spectrogram and Mel-spectrogram from the original waveform. In each spectrogram, the patches are first sampled along the time axis and then the frequency axis so that each patch maintains the locality in time to a maximal extent. We then concatenate patches from different resolutions within the same window. Each patch is equipped with a disentangled positional encoding similar to \cite{koutini2021efficient}, i.e, we generate individual encoding vectors in time, frequency and resolution, and add them to the patches. The patches are then sent to a hierarchical structure consisting of Patch-Merge Layers and SWIN Transformer Blocks\cite{liu2021swin} as shown in Figure~\ref{fig:training}. Note that although we expand the input from a single spectrogram to a set of spectrograms in different resolutions, the computational complexity is not changed due to the window mechanism. 

% \noindent\textbf{Acoustic Attention: Multi-filter along Heads.} 


% \noindent\textbf{Acoustic Attention: Multi-resolution along sequence} 


% \noindent\textbf{Multi-scale Patch Embedding.} 

==> tex_img_tab/SCM.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\columnwidth]{images/SCM-cropped.pdf}
    \caption{SCM TODO: fillin}
    \label{fig:scm}
\end{figure}

==> tex_img_tab/multi-filter.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\columnwidth]{images/multi-filter.pdf}
    \caption{multi-filtered spectrograms across different attention heads}
    \label{fig:multi-filter}
\end{figure}

==> tex_img_tab/multi-resolution.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\columnwidth]{images/multi-resolution.pdf}
    \caption{multi-resolution across heads: we sample from the input waveform using different resolutions, and match the dimension with a linear transformation. }
    \label{fig:multi-resolution}

\end{figure}

==> tex_img_tab/tab_ablation_MRMF.tex <==
\begin{table}[!htbp]
  \caption{\textit{Ablation study on the Multi-Resolution Multi-Filter (MRMF) and causal designs. We isolated each part of the design and compare them on both CAT model (ours) and AST model, and evalutated on ESC50.} }
  \vspace{-.6cm}
  \label{tab:ablation}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{l c c}
    \toprule
    \textbf{Models} & \textbf{Accuracy} & \text{Pretrain} \\
    \midrule
    \thead{CAT }    & 96.4\%    &  ImageNet and Audio Set    \\  
    \thead{CAT no causal}    &  95.9\%   &  ImageNet and Audio Set  \\ 
    \midrule
    \thead{CAT from scratch }  & 89.4\%    &  -    \\  
    \thead{CAT from scratch no causal} & 88.7\%  & -\\
    \midrule
    \thead{AST\cite{gong2021ast} from scratch }  & 88.7\%    &  -    \\  
    \thead{AST + MRMF } & 88.9\%  & -\\
    \thead{AST + causal } & 89.1\%  & -\\   
  \bottomrule
\end{tabular}
}%resize box ends here
\end{table}

==> tex_img_tab/tab_causal.tex <==
\begin{table}[!htbp]
  \caption{\textit{We tested CAT on ESC50 and UrbanSound8K (US8K) for robustness in its transferability. } }
  \vspace{-.6cm}
  \label{tab:ablation}
  \resizebox{\columnwidth}{!}{%
  \centering
  \begin{tabular}{lccc}
    \toprule
    \textbf{Models} & \textbf{Accuracy} & \textbf{Pretrain} & \textbf{Evaluation Set}\\
    \midrule
    \thead{CAT no causal}    & 95.9\%    & US8K & ESC50    \\  
    \thead{CAT no causal}    &  84.1\%   & ESC50 & US8K  \\ 
    \midrule
    \thead{CAT  }  & 96.1\%   & US8K & ESC50   \\  
    \thead{CAT }   & 86.7\%    & ESC50 & US8K\\
  \bottomrule
\end{tabular}
}%resize box ends here
\end{table}

==> tex_img_tab/tab_esc50.tex <==
\begin{table}[!htbp]
  \caption{Evaluation on AudioSet}
  \vspace{-.6cm}
  \label{tab:esc50}
  \centering
  \resizebox{.9\columnwidth}{!}{%
  \begin{tabular}{cccc}
    \toprule
    \textbf{Models}  & \textbf{ensemble} & \textbf{accuracy} & \textbf{note} \\
    \midrule
    \thead{HTS-AT \cite{chen2022hts}}               & Y      & 97.0\%    & - \\
    \thead{CLAP \cite{elizalde2022clap}}            & -      & 96.7\%    & language supervision\\
    \thead{\cite{zhao2021connecting}}               & -      & 95.7\%    & visual supervision\\
    \thead{AST \cite{gong2021ast}}                  & Y      & 95.7\%    & -\\
    \midrule
    \thead{ours}                                    & N      & 96.4\%    & -\\
    \thead{ours no causal}                          & N      & 95.9\%    & - \\
    \thead{ours train from scratch}                                    & N      & 88.7\%    & -\\
  \bottomrule
\end{tabular}
}%resize box ends here
\end{table}
